How Does Gender Balance In Training Data Affect Face Recognition Accuracy?

Deep learning methods have greatly increased the accuracy of face recognition, but an old problem still persists: accuracy is usually higher for men than women. It is often speculated that lower accuracy for women is caused by under-representation in the training data. This work investigates female under-representation in the training data is truly the cause of lower accuracy for females on test data. Using a state-of-the-art deep CNN, three different loss functions, and two training datasets, we train each on seven subsets with different male/female ratios, totaling forty two trainings, that are tested on three different datasets. Results show that (1) gender balance in the training data does not translate into gender balance in the test accuracy, (2) the "gender gap" in test accuracy is not minimized by a gender-balanced training set, but by a training set with more male images than female images, and (3) training to minimize the accuracy gap does not result in highest female, male or average accuracy

==> figures/cluster_full.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{M C}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/morph_c_softmax.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \caption{M AA}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_softmax.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \caption{ND}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_softmax.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \caption{IJB-B}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_softmax.png}
        \end{subfigure}
        \vspace{-0.5em}
        \addtocounter{subfigure}{-4}
        \caption{Softmax}
        \vspace{-0.5em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{.215\textwidth}
            \caption{M C}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_combined.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \caption{M AA}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/morph_aa_combined.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{ND}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/ours_combined.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{IJB-B}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/ijbb_combined.png}
        \end{subfigure}
        \vspace{-0.5em}
        \caption{Combined Margin}
        \vspace{-0.5em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{M C}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/morph_c_triplet.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{M AA}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/morph_aa_triplet.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{ND}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/ours_triplet.png}
        \end{subfigure}
        \begin{subfigure}[b]{.215\textwidth}
            \centering
            \caption{IJB-B}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/ijbb_triplet.png}
        \end{subfigure}
        \vspace{-0.5em}
        \caption{Triplet}
        \vspace{-0.5em}
    \end{subfigure}
    \caption{Features for the MORPH Caucasians (M C), MORPH African American (M AA), Notre Dame (ND), and IJB-B datasets clustered into two groups: inner and outer circles represent the two clusters. Males in blue, and females in red.}
    \vspace{-1.5em}
    \label{fig:clusters}
\end{figure*}

==> figures/clusters.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{.48\textwidth}
        \begin{subfigure}[b]{.32\textwidth}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_softmax.png}
            \caption{Softmax}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_combined.png}
            \caption{Comb. Margin}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_triplet.png}
            \caption{Triplet}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{MORPH Caucasian}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{.48\textwidth}
        \begin{subfigure}[b]{.32\textwidth}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_softmax.png}
            \caption{Softmax}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_combined.png}
            \caption{Comb. Margin}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_triplet.png}
            \caption{Triplet}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{MORPH African American}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{.48\textwidth}
        \begin{subfigure}[b]{.32\textwidth}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_softmax.png}
            \caption{Softmax}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_combined.png}
            \caption{Comb. Margin}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_triplet.png}
            \caption{Triplet}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{Ours}
        \vspace{-0.5em}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{.48\textwidth}
        \begin{subfigure}[b]{.32\textwidth}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_softmax.png}
            \caption{Softmax}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_combined.png}
            \caption{Comb. Margin}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.32\textwidth}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_triplet.png}
            \caption{Triplet}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{IJB-B}
        \vspace{-0.5em}
    \end{subfigure}
    \caption{Features clustered into two groups: inner and outer circles represent the two clusters. Males in blue, and females in red.}
    \vspace{-1em}
    \label{fig:clusters}
\end{figure*}

==> figures/clusters_new.tex <==
\begin{figure}[t]
    \begin{subfigure}[b]{1\columnwidth}
        \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{.225\textwidth}
            %\renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \caption{MORPH C}
            \vspace{-0.5em}
            \includegraphics[width=1\columnwidth]{images/morph_c_softmax.png}
            %\caption{\scriptsize{MORPH C}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}2}
            \caption{MORPH AA}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_softmax.png}
            %\caption{\scriptsize{MORPH AA}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}3}
            \caption{Notre Dame}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_softmax.png}
            % \caption{\scriptsize{Notre Dame}}
            % \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}4}
            \caption{IJB-B}
            \vspace{-0.5em}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_softmax.png}
            % \caption{\scriptsize{IJB-B}}
            % \vspace{-0.5em}
        \end{subfigure}
        %\addtocounter{subfigure}{-1}
        \vspace{-0.5em}
        \addtocounter{subfigure}{-4}
        \caption{Softmax}
    \end{subfigure}
    
    \begin{subfigure}[b]{1\columnwidth}
        \begin{subfigure}[b]{.225\textwidth}
            %\renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_combined.png}
            %\caption{\scriptsize{MORPH C}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %\addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_combined.png}
            % \caption{\scriptsize{MORPH AA}}
            % \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_combined.png}
            % \caption{\scriptsize{Notre Dame}}
            % \vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}4}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_combined.png}
            %\caption{\scriptsize{IJB-B}}
            %\vspace{-0.5em}
        \end{subfigure}
        %%\addtocounter{subfigure}{-1}
        \vspace{-0.5em}
        \caption{Combined Margin}
    \end{subfigure}
    
    \begin{subfigure}[b]{1\columnwidth}
        \begin{subfigure}[b]{.225\textwidth}
            %\renewcommand\thesubfigure{\alph{subfigure}1}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_c_triplet.png}
            %\caption{\scriptsize{MORPH C}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}2}
            \centering
            \includegraphics[width=1\columnwidth]{images/morph_aa_triplet.png}
            %\caption{\scriptsize{MORPH AA}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}3}
            \centering
            \includegraphics[width=1\columnwidth]{images/ours_triplet.png}
            %\caption{\scriptsize{Notre Dame}}
            %\vspace{-0.5em}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.225\textwidth}
            %%\addtocounter{subfigure}{-1}
            %\renewcommand\thesubfigure{\alph{subfigure}4}
            \centering
            \includegraphics[width=1\columnwidth]{images/ijbb_triplet.png}
            %\caption{\scriptsize{IJB-B}}
            %\vspace{-0.5em}
        \end{subfigure}
        %%\addtocounter{subfigure}{-1}
        \vspace{-0.5em}
        \caption{Triplet}
        \vspace{-0.5em}
    \end{subfigure}
    \caption{Features clustered into two groups: inner and outer circles represent the two clusters. Males in blue, and females in red.}
    \vspace{-1.5em}
    \label{fig:clusters}
\end{figure}

==> figures/ms1mv2_subsets.tex <==
\begin{table}[t]
    \centering
    \small
    %\setlength\tabcolsep{4.5pt}
    \begin{tabular}{l|rr|rr}
        \textbf{}& \multicolumn{2}{c|}{\textbf{\# Subjects}}& \multicolumn{2}{c}{\textbf{\# Images}} \\
        \textbf{Subset Name} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c|}{\textbf{Females}} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c}{\textbf{Females}} \\ \hline
        Full & 59,563 & 22,499 & 3,741,274 & 1,890,773\\
        Balanced & 22,499 & 22,499 & 1,890,773 & 1,890,773\\ \hline
        F100 & 0 & 22,499 & 0 & 1,890,773\\
        M25F75 & 5,624 & 16,875 & 472,693 & 1,418,080\\
        M50F50 & 11,249 & 11,249 & 945,386 & 945,386\\
        M75F25 & 16,875 & 5,624 & 1,418,080 & 472,693\\
        M100 & 22,499 & 0 & 1,890,773 & 0 
    \end{tabular}
    \caption{MS1MV2 training subsets created.}
    \vspace{-1em}
    \label{tab:training_datasets_ms1mv2}
\end{table}

==> figures/subsets.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \setlength\tabcolsep{2pt}
        \begin{tabular}{l|rr|rr|rr|rr}
         & \multicolumn{4}{c|}{\textbf{VGGFace2}} & \multicolumn{4}{c|}{\textbf{MS1MV2}} \\
        \textbf{} & \multicolumn{2}{c|}{\textbf{\# Subjects}} & \multicolumn{2}{c|}{\textbf{\# Images}} & \multicolumn{2}{c|}{\textbf{\# Subjects}} & \multicolumn{2}{c|}{\textbf{\# Images}} \\
        \textbf{Subset} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c|}{\textbf{Females}} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c|}{\textbf{Females}} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c|}{\textbf{Females}} & \multicolumn{1}{c}{\textbf{Males}} & \multicolumn{1}{c}{\textbf{Females}} \\ \hline
        Full & 5,154 & 3,477 & 1,828,987 & 1,291,873 & 59,563 & 22,499 & 3,741,274 & 1,890,773 \\
        Balanced & 3,477 & 3,477 & 1,291,873 & 1,291,873 & 22,499 & 22,499 & 1,890,773 & 1,890,773 \\ \hline
        M50F50 & 1,739 & 1,739 & 645,937 & 645,937 & 0 & 22,499 & 0 & 1,890,773 \\
        M75F25 & 2,607 & 870 & 968,904 & 322,969 & 5,624 & 16,875 & 472,693 & 1,418,080 \\
        M25F75 & 870 & 2,607 & 322,969 & 968,904 & 11,249 & 11,249 & 945,386 & 945,386 \\
        F100 & 0 & 3,477 & 0 & 1,291,873 & 16,875 & 5,624 & 1,418,080 & 472,693 \\
        M100 & 3,477 & 0 & 1,291,873 & 0 & 22,499 & 0 & 1,890,773 & 0
        \end{tabular}
        \vspace{-0.5em}
    \caption{VGGFace2 and MS1MV2 training subsets created.}
    \vspace{-1em}
    \label{tab:training_datasets}
\end{table}

==> figures/vggface2_test_results.tex <==
\begin{table*}[ht]
    \setlength\tabcolsep{4pt}
    \centering
    % \ra{1.3}
    \begin{tabular}{rrrrrrrrrrrrr}
        \multicolumn{1}{l}{} & & \multicolumn{3}{c}{\textbf{Softmax Loss}} & & \multicolumn{3}{c}{\textbf{CM Loss}} & & \multicolumn{3}{c}{\textbf{Triplet Loss}} \\
        \textbf{Training Data} & & \textbf{Males} & \textbf{Females} & \textbf{All Data} & & \textbf{Males} & \textbf{Females} & \textbf{All Data} & & \textbf{Males} & \textbf{Females} & \textbf{All Data} \\ \hline
        Full dataset & & 4.17 & 4.99 & 4.67 & & 6.15 & 6.48 & 6.52 & & & & \\
        Dataset balanced & & \textbf{4.08} & \textbf{4.56} & \textbf{4.41} & & \textbf{5.79} & \textbf{5.75} & \textbf{5.95} & & & & \vspace{0.75em}\\
        50\% males 50\% females & & 4.99 & 5.42 & \textbf{5.34} & & 8.71 & \textbf{8.68} & 9.04 & & & & \\
        75\% males 25\% females & & 4.51 & 6.25 & 5.41 & & \textbf{7.6} & 9.31 & \textbf{8.58} & & & & \\
        25\% males 75\% females & & 5.64 & \textbf{5.1} & 5.6 & & 11.99 & 11.36 & 12.28 & & & & \\
        Females only & & {\color[HTML]{CB0000} \textbf{8.77}} & 5.28 & {\color[HTML]{CB0000} \textbf{7.69}} & & {\color[HTML]{CB0000} \textbf{18.32}} & 11.25 & {\color[HTML]{CB0000} \textbf{16.17}} & & & & \\
        Males only & & \textbf{4.31} & {\color[HTML]{CB0000} \textbf{9.41}} & 6.64 & & 8.29 & {\color[HTML]{CB0000} \textbf{13.77}} & 10.89 & & & &
    \end{tabular}
    \caption{Top-1 classification error (\%) on VGGFace2 test set.}
    \label{tab:vggface2_test}
\end{table*}
